FoAR: Force-Aware Reactive Policy for Contact-Rich Robotic Manipulation

Contact-rich tasks present significant challenges for robotic manipulation policies due to the complex dynamics of contact and the need for precise control. Vision-based policies often struggle with the skill required for such tasks, as they typically lack critical contact feedback modalities like force/torque information. To address this issue, we propose FoAR, a force-aware reactive policy that combines high-frequency force/torque sensing with visual inputs to enhance the performance in contact-rich manipulation. Built upon the RISE policy, FoAR incorporates a multimodal feature fusion mechanism guided by a future contact predictor, enabling dynamic adjustment of force/torque data usage between non-contact and contact phases. Its reactive control strategy also allows FoAR to accomplish contact-rich tasks accurately through simple position control. Experimental results demonstrate that FoAR significantly outperforms all baselines across various challenging contact-rich tasks while maintaining robust performance under unexpected dynamic disturbances. Project website: https://tonyfang.net/FoAR/

==> 5_analysis.tex <==
\red{\section{Limitation and Future Work}}

\red{While FoAR demonstrates significant advancements in contact-rich robotic manipulation, it faces several key limitations.} 
%\red{One key limitation lies in its reliance on force/torque sensing, which, compared to tactile sensing, lacks the ability to provide precise contact position information or detailed object-contact patterns. Additionally,}
\red{One limitation lies in the use of static force/torque thresholds. Though effective in the evaluated tasks, this static setting may not generalize well to scenarios with varying object properties or environmental conditions.}

\red{The policy's reliance on position control limits its ability to handle tasks requiring precise force regulation like assembling delicate components. Future work could address this by integrating advanced control strategies like hybrid force/position control to further enhance the versatility of the policy.}

